Shaping the distribution of neural responses with interneurons in a recurrent circuit model

Efficient coding theory posits that sensory circuits transform natural signals into neural representations that maximize information transmission subject to resource constraints. Local interneurons are thought to play an important role in these transformations, dynamically shaping patterns of local circuit activity to facilitate and direct information flow. However, the relationship between these coordinated, nonlinear, circuit-level transformations and the properties of interneurons (e.g., connectivity, activation functions, response dynamics) remains unknown. Here, we propose a normative computational model that establishes such a relationship. Our model is derived from an optimal transport objective that conceptualizes the circuit's input-response function as transforming the inputs to achieve an efficient target response distribution. The circuit, which is comprised of primary neurons that are recurrently connected to a set of local interneurons, continuously optimizes this objective by dynamically adjusting both the synaptic connections between neurons as well as the interneuron activation functions. In an example application motivated by redundancy reduction, we construct a circuit that learns a dynamical nonlinear transformation that maps natural image data to a spherical Gaussian, significantly reducing statistical dependencies in neural responses. Overall, our results provide a framework in which the distribution of circuit responses is systematically and nonlinearly controlled by adjustment of interneuron connectivity and activation functions.

==> rebuttal.tex <==
\newcommand{\eero}[1]{{\color{ForestGreen}EPS: #1}}
\newcommand{\rebuttal}[1]{{\color{Plum} #1}}
\newcommand{\david}[1]{{\color{RubineRed}DL: #1}}

\section{Rebuttals}

\subsection{General response}

\rebuttal{
We thank the reviewers for their careful reading of our work and for their helpful comments. We have revised our paper in accordance with the reviewers' suggestions and provide individual responses to their comments. Here we respond to two important concerns raised by the reviewers.
\paragraph{Biological plausibility.} Reviewers {\bf zp8S}, {\bf Voaj} and {\bf txmi} listed the biological realism of our model as a primary concern that limits the applicability of our model in understanding neural circuits. 
We appreciate the reviewers' concerns, though we do not believe they significantly limit the usefulness of our model.

First, several of the reviewers' concerns regarding biological realism can be readily addressed with minor adjustments that do not affect the circuit computation.
We enumerate these as follows:
\begin{enumerate}
    \item {\bf Dale's law.} Algorithm 1 does not sign-constrain the weight matrix $\rmW$, so it violates Dale's law in the current circuit implementation.
    This is the most serious concern (though Dale's law may not be as hard of a constraint as previously thought; see Saunders et al.~2016 and Granger et al.~2020).
    There are two possible solutions to this problem.
    One approach is to seek a circuit implementation of the algorithm that obeys Dale's law.
    This could potentially be achieved by introducing additional (excitatory or inhibitory) neural populations, though it is not immediately clear how.
    An alternative approach is to replace the current optimization problem with a \textit{constrained} optimization problem that respects Dale's law and can be optimized via a projected gradient descent algorithm.
    To test the efficacy, we optimized the constrained optimization problem (in the fully online setting with batch size one) and find that the solution significantly reduces the mutual information between neural responses, though not as much as the unconstrained optimization problem.
    \item {\bf Batch training.} Using a batch size 10 was an optimization choice and is not required. We could have implemented a fully online optimization algorithm with batch size 1. To demonstrate this, we ran Algorithm 1 in the fully online setting and reproduced Figure 3B of the main text (for one image due to time constraints); see Figure \ref{fig:online} of the attached PDF. 
    \item {\bf Symmetry of synaptic weights.} While Algorithm 1 enforces symmetry between the primary neuron-to-interneuron weights $\rmW^\top$ and interneuron-to-primary neuron weights $-\rmW$, this is not required.
    When the weights are decoupled, they will asymptotically converge to be symmetric due to the symmetry of their Hebbian (anti-Hebbian) learning rules.
    This has been demonstrated both analytically and numerically in previous works; see, e.g, \citep[appendix E.2]{duong2023adaptive}.
    \item {\bf Wavelet coefficients.} Wavelet coefficient are responses of a spatially local oriented filter (similar to a Gabor filter) applied to natural images. These responses are qualitatively similar to simple cell responses in primary visual cortex \citep{field1987relations}, so they are representative of natural inputs to cortical circuits in the visual cortex. We don't think ``wavelet coefficients'' was an apt description within the context of this work, so we will edit the text and refer to the inputs as ``local filter responses''.
\end{enumerate}

Second, even though there are aspects of our model that are not biologically realistic, we believe that our normative model strikes an effective balance between simplicity and biological realism that is useful for interpreting experimental measurements of neural circuits.
Our model suggests a novel framework for interpreting experimental measurements.
Specifically, our model suggests the following experimental measurements:
\begin{enumerate}
    \item Our model conceptualizes the circuit computation as transforming the input distribution to achieve a target distribution (or set of distributions).
    This can potentially be experimentally tested by measuring distributions of circuit responses (and how these change when the input distribution shifts).
    We think this is especially useful when recording from large populations of neurons and there is some work along these lines (Bennucci et al.~2013).
    \item We establish a link between the circuit level computation and different adaptation mechanisms at the physiological level. This can be experimentally tested by measuring if FI curves in interneurons adapt in response to changes in the distribution of circuit inputs.
\end{enumerate}

\paragraph{Existing work.}
Reviewer {\bf Voaj} pointed out that our original submission does not cite salient works related to circuit models that implement nonlinear transformations to efficiently encode information.
We take this point quite seriously and in our revision we plan to better place our work in the context of related works by adding the following discussion:
\begin{quote}
    There are a number of existing normative models that explain how neural circuits can implement nonlinear transformations to efficiently encode their inputs.
    For example, there are several neural circuit models that implement forms of divisive normalization \citep{rubin2015stabilized,chalk2017sensory,heeger2020recurrent,malo2024cortical}, a transformation that is optimal for efficient encoding of natural signals \citep{schwartz_natural_2001,lyu2011dependency,chalk2017sensory}.
    In addition, there are many normative spiking models that are derived from efficient coding objectives with metabolic costs on spikes \citep{koren2017computational,gutierrezpopulation2019}.

    Our model differs from these existing works in fundamental aspects.
    First, we frame the problem in terms of a transformation of probability distributions.
    This can be viewed as a population level extension of the work by Laughlin 1981, which considers this problem at the level of a single neuron.
    Second, we propose that this objective can be effectively optimized by reshaping a select number of marginal distributions.
    Third, we demonstrate in a normative circuit model how interneurons can play a critical role by both measuring and reshaping the marginal distributions of the primary neuron population.
\end{quote}
}

\subsection{Reviewer zp8S: 4(2)}

\subsubsection*{Weaknesses}
\begin{enumerate}
    \item A main concern is that the model is not biologically realistic. In addition to the authors' admission that the feedforward synaptic weights $W^T$ and feedback weights $-W$ are symmetrically constrained, there is also a question about the biological plausibility of using pairs of wavelet coefficients as inputs. It's unclear how biological systems would naturally derive such information and whether the distribution of these inputs is something that biological systems need to transform.

    \rebuttal{First, we could implement this algorithm exactly while following Dale's law. This would require incorporating additional neural populations. Alternatively, we can modify our existing algorithm, effectively transforming it to a constrained optimization problem.}
    \item The setup of online learning with a batch size of 10 also raises questions about its biological feasibility. It's uncertain how biological systems could implement a similar mechanism.
    
    \rebuttal{This is simply a choice for efficient optimization purposes and does not affect the optimal solution. In Figure \ref{fig:online}, we show that we can obtain comparable results with a batch size of 1.}
    \item The paper only demonstrates the method's effectiveness on two-dimensional inputs, which might not sufficiently prove its efficacy. In real-world scenarios, we often deal with inputs that are high-dimensional ($N\gg2$), and the model's performance in such conditions remains untested.
    
    \rebuttal{This is an important point worth further investigation. We have strong reason to believe that the network will scale with the number of inputs. For example, visual inputs are highly structured with statistical dependencies rapidly decaying with the distance between pixels. Therefore, while the input may be high-dimensional, the input to a single neuron is statistically independent from most of the neural population's inputs.}
    \item The paper incorporates many specific settings, such as the choice of activation functions based on the Gaussianization of scalar signals. These particular choices may limit the generalizability and applicability of the model to different datasets or broader applications.

    \rebuttal{While the specific example incorporated specific choices, these choices were informed by the statistical properties of the inputs. In particular, the activation function was chosen to match the statistics of the inputs. This provides a systematic method for choosing the activation functions which we believe \textit{facilitates} the generalizability of the model.}
\end{enumerate}

\subsubsection*{Questions}
\begin{enumerate}
    \item  As mentioned in the Weaknesses section, the model is not biologically realistic. Given this, my primary question is: What is the purpose of using neural networks to implement this function? Furthermore, if it does not realistically mimic biological processes, should it be compared with more engineering-oriented approaches?
    
    \rebuttal{While there are aspects of our circuit that do not match biology, we believe our model is useful for understanding biological circuits. 
    Our model matches many aspects of biological circuits (local learning rules, online learning, separate neural populations). 
    Our model provides a unified objective from which synaptic plasticity, gain modulation and activation function adjustments naturally emerge from optimization of the objective. For example, our model suggests a novel perspective for thinking about certain local interneurons as measuring the marginal statistics of primary neuron responses and adjusting their response properties accordingly. This could potentially lead to experiments that test whether local interneurons adapt their gain and activation functions when their input statistics change. Importantly, our model provides a novel perspective for thinking about circuits in the context of transformations of distributions.}
    \item Scaling of Inhibitory Neurons with Input Dimensionality: The model currently demonstrates with two-dimensional inputs, requiring three inhibitory neurons. How does the number of required inhibitory neurons scale as the dimensionality of the input increases? This is crucial for understanding the feasibility and complexity of the model when applied to higher-dimensional data.
    
    \rebuttal{This is an important point! It is of primary interest to understand how the model scales with the dimension of the input. We have strong reason to believe that the number of inhibitory interneurons will scale reasonably with the dimension of the input. For example, as mentioned above, in the case of visual inputs, the statistical dependencies between inputs rapidly decay with the distance between the inputs (e.g., receptive fields that are far from each other are effectively statistically independent). Therefore, local interneurons only need to connect to neurons with overlapping or adjacent receptive fields, which greatly reduces the number of interneurons that are required.}
\end{enumerate}

\subsection{Reviewer Voaj: 4(3)}

\subsubsection*{Weaknesses}
The paper has the ambition of finding a neural implementation of generalized whitening such that it could be also implemented by biological neural circuits. However, a major concern is that inhibitory neurons do not obey Dale's law, and the model is therefore not biologically plausible. In general, it is not clear what the paper brings to understanding of biological or artificial neural networks. Since the model violates Dale's law, the discussion about the function of interneurons seems out of scope.

\rebuttal{We can implement the algorithm in a circuit that obeys Dale's law. Alternatively, we can implement a constrained version of the algorithm with the same architecture.}

Moreover, there are significant parts of the paper that are unclear. A number of details about the methods are given, but the main mechanism that supports learning remains unclear. Authors mention that the circuit "learns directions that are least matched to the target distribution", but it remained unclear to me how is this achieved and why this helps to Gaussianize the distribution of output firing rates of principal neurons.

\rebuttal{We will improve the clarity.}

Authors motivate their model by claiming that divisive normalization has not yet been solved with a neural network. This seems false (see for example Chalk, Masset, Deneve \& Gutkin, PLOS CB 2017). Gain control is also captured by available models. Efficient spiking models and normative models where changes in gain control can be captured by modulating the metabolic cost on spiking in the model's objective (see Guiterrez and Deneve, eLife 2019; Koren and Deneve, PLOS CB 2017). In general, the paper does not sufficiently take into account previous work on efficient coding with spikes that is closely related.

\rebuttal{Thank you for pointing out these omissions. We take your point quite seriously and acknowledge that we did not properly credit many existing neural circuit models that implement nonlinear transformations related to efficient coding nor explain how our model differs from these works. 
In our revision, we plan to add the following discussion that places our work within the context of existing circuit models that perform nonlinear transformations related to efficient coding.

\begin{quote}
There are a number of existing computational models that explain how neural circuit can perform nonlinear transformations to efficiently encode their inputs.

Neural implementations of divisive normalization:
In one line of work, the parameters of physiological models of neural circuits are matched to nonlinear phenomenological models such as divisive normalization that have been shown to improve the efficiency of the neural code by reducing redundancy \citep{rubin2015stabilized,chalk2017sensory,heeger2019oscillatory,heeger2020recurrent,malo2024cortical}.

Efficient spiking models and normative models where changes in gain control can be captured by modulating the metabolic cost on spiking in the model's objective (see Guiterrez and Deneve, eLife 2019; Koren and Deneve, PLOS CB 2017).

Alemi et al.~(2018) propose a spiking network that implements a nonlinear transformation with (i) local synaptic plasticity rules, (ii) reduced redundancy and (iii) robust to noise and loss of neurons.
The nonlinear transform corresponds to learning a nonlinear dynamical system (student-teacher framework) with L1 and L2 penalties on the firing rates.

Koren \& Panzeri (2022) propose E-I spiking networks that maximize information transmission.
Desired circuit output is a \textbf{linear} transformation of the input.
\end{quote}

}

There are typos on several places, for example: lines 75, 77, 100, 234

\rebuttal{Thank you for pointing us to these typos, we will correct them.}

\subsubsection*{Questions}
\begin{enumerate}
\item  Authors motivate their modelling by claiming that it is currently unclear how neural networks could implement nonlinear transformations. Which non-linear transformations are not captured by the listed models? The paper by Alemi et al. AAAI 2018, proposes efficient spiking models that implement non-linear transformation of stimuli at the population level. In Koren \& Panzeri, NeurIPS 2022, neural populations perform linear transformation of stimuli on the level of neural populations, but on the level of single neurons these transformations are strongly non-linear. What do authors mean by non-linear transformations? Non-linear on what level? This should be clarified.
\item Authors say that approximating target distribution is useful because it facilitates efficient transmission of signals. It is however not entirely clear why making the distribution of responses Gaussian-like facilitates efficient transmission. Is this improvement in efficient transmission attributed to redundancy reduction?

\rebuttal{Yes, it is primary attributed to redundancy reduction. However, there are also other reasons to believe Gaussian distributions facilitate information transmission. For example, if metabolic costs are proportional to the variance of the neural responses, then the Gaussian distribution maximizes information transmission subject to a metabolic constraint. In addition, there is experimental evidence that LMC neurons in the early fly visual system Gaussianize their responses (Van Hateren 1997).}

\item Is inhibition required to solve this optimization problem, e.g., could the same operation be achieved through plasticity of E neurons?

\rebuttal{It is likely that plasticity of excitatory neurons can contribute to reshaping of neural responses; however, redundancy reduction likely requires local inhibitory interneurons. For example, we are unaware how plasticity of EE connections can reduce correlations between two primary neuron responses that receive highly correlated inputs.}
\end{enumerate}

\subsection{Reviewer 3 txmi: 5(2)}

Note: As I am not well-versed in wavelet transformations, which are extensively utilized in the experimental section, my review focuses primarily on the theoretical aspects prior to the experiments (Section 4).

\rebuttal{Wavelet transformations are spatially localized linear filters similar to Gabor filters. The filter responses are qualitatively similar to simple cell responses in the primate visual cortex.}

\subsubsection*{Weaknesses}

\begin{enumerate}
    \item The authors should define $p_\text{target}$, $p_\text{marginal}$, and $p_r$ explicitly instead of using descriptive terms for better clarity.
    
    \rebuttal{We will explicitly define these distributions for improved clarity.}
    \item The proposed model necessitates different $g$, $\theta$ and $w$ for different stimuli. While neurons can potentially adjust their gain and activation function (i.e., $g$, $\theta$) relatively quickly, the need for weight updates to handle varying inputs significantly limits the model's applicability and biological plausibility.
    
    \rebuttal{This is a great point. Interestingly, the learned weights are approximately shared across images, whereas the optimal $g$ and $\theta$ vary between images. This is consistent with rapid adjustments of $g$ and $\theta$ and slow adjustments of $\rmW$. We did focus on this point because Duong et al.\ 2023 have shown similar results. Specifically, they showed how a multi-timescale circuit with fast gain adjustments and slow synaptic updates can effectively (linearly) whiten circuit responses to changing contexts. Here, our focus is on the nonlinear aspects of the circuit; however, we will add a discussion of this in our revision.}
    \item As noted in the limitations section, the weights are not sign-constrained. Therefore the distinguishing between excitatory and inhibitory neurons in this model makes no sense.
    
    \rebuttal{They are distinguished by their connectivity patterns. Also, we can sign constrain the weights and everything works...}
\end{enumerate}

\subsubsection*{Questions}

\begin{enumerate}
\item The constraint $g_i>0$ is not included in Algorithm 1. Would imposing these constraints ($w>0$, $g>0$)  negatively impact the experimental results?

\rebuttal{We tested a constrained version of our results and find that there is a slight degradation in the performance; however, the model still performs very well.}

\end{enumerate}


\subsubsection*{Limitations}
The authors have adequately addressed the limitation.

\subsection{Reviewer DTUH: 8(4)}

\subsubsection*{Weaknesses}
I have only a few small concerns regarding the biological realism of the model, but these are mostly already acknowledged by the authors. One point that I believe warrants further discussion is the plausibility of the activation functions (6). These are somewhat reminiscent of two-sided versions of the rectified-power law activations used in cortical models, no? I also have a handful of miscellaneous questions (see below), but on the whole these do not dampen my enthusiasm.

\rebuttal{Indeed, the activation functions in (6) resemble two-sided versions of the rectified-power law activations.
One interesting aspect of our model is that it suggests a relationship between the interneuron activation functions and the primary neuron responses. FILL IN.}

\subsubsection*{Questions}
\begin{enumerate}
    \item Along with the work of Van Hateren, the authors might consider citing Laughlin, "A simple coding procedure enhances a neuron's information capacity," and Juusola and Hardie, "Light Adaptation in Drosophila Photoreceptors." I leave it to their discretion whether or not to do so.

    \rebuttal{Thank you for the suggestion, we will include references to these works in our revision.}
    \item In that vein, it might be nice to provide further evidence for adaptation of activation functions in biology. If additional references occur to me, I will update my review.
    
    \rebuttal{Thank you! We will also add a reference to Sharpee et al.~2006, which demonstrates that neurons in cat primary visual cortex adapt to higher-order statistics beyond mean and covariance.}
    \item In Line 271, should "activations" be plural? I think this is a typo.
    
    \rebuttal{We will correct this typo.}
    \item The legibility of Figure 3A could be improved; as it stands the text is a bit too small and the lines a bit too faint.

    \rebuttal{We will increase the legibility of Figure 3A.}
    \item It could be nice to provide further support for the approximate form of the activation functions. Can you numerically evaluate the expression below Line 630?

    \rebuttal{Yes, these are the thick gray curves in Figure 2C. We will add text below Line 630 pointing to Figure 2C.}
\end{enumerate}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/rebuttal/mutual_info (2).pdf}
    \caption{For spatial offsets between $d=2$ and $d=64$, the estimated mutual information (using bin size 0.5) of the inputs (generated from a single image), the ZCA whitened input, the learned circuit responses with $K=3$ and Dale's law violated, and the learned circuit responses with $K=3$ and Dale's law enforced. The circuit responses were computed after $10^6$ iterations in the fully online setting (i.e., batch size 1).}
    \label{fig:MI}
\end{figure}
